Prompt charm production in pp collisions at sqrt(s)=7 TeV

Charm production at the LHC in pp collisions at sqrt(s)=7 TeV is studied with the LHCb detector. The decays D0 -> K- pi+, D+ -> K- pi+ pi+, D*+ -> D0(K- pi+) pi+, D_s+ -> phi(K- K+) pi+, Lambda_c+ -> p K- pi+, and their charge conjugates are analysed in a data set corresponding to an integrated luminosity of 15 nb^{-1}. Differential cross-sections dsigma/dp_T are measured for prompt production of the five charmed hadron species in bins of transverse momentum and rapidity in the region 0 < p_T < 8 GeV/c and 2.0 < y < 4.5. Theoretical predictions are compared to the measured differential cross-sections. The integrated cross-sections of the charm hadrons are computed in the above p_T-y range, and their ratios are reported. A combination of the five integrated cross-section measurements gives sigma(c\bar{c})_{p_T < 8 GeV/c, 2.0 < y < 4.5} = 1419 +/- 12 (stat) +/- 116 (syst) +/- 65 (frag) microbarn, where the uncertainties are statistical, systematic, and due to the fragmentation functions.

==> LHCb_comma_separated_author.tex <==
LHCb collaboration:
R. Aaij, 
C. Abellan Beteta, 
A. Adametz, 
B. Adeva, 
M. Adinolfi, 
C. Adrover, 
A. Affolder, 
Z. Ajaltouni, 
J. Albrecht, 
F. Alessio, 
M. Alexander, 
S. Ali, 
G. Alkhazov, 
P. Alvarez Cartelle, 
A.A. Alves Jr, 
S. Amato, 
Y. Amhis, 
L. Anderlini, 
J. Anderson, 
R. Andreassen, 
R.B. Appleby, 
O. Aquines Gutierrez, 
F. Archilli, 
A. Artamonov , 
M. Artuso, 
E. Aslanides, 
G. Auriemma, 
S. Bachmann, 
J.J. Back, 
C. Baesso, 
V. Balagura, 
W. Baldini, 
R.J. Barlow, 
C. Barschel, 
S. Barsuk, 
W. Barter, 
Th. Bauer, 
A. Bay, 
J. Beddow, 
I. Bediaga, 
S. Belogurov, 
K. Belous, 
I. Belyaev, 
E. Ben-Haim, 
M. Benayoun, 
G. Bencivenni, 
S. Benson, 
J. Benton, 
A. Berezhnoy, 
R. Bernet, 
M.-O. Bettler, 
M. van Beuzekom, 
A. Bien, 
S. Bifani, 
T. Bird, 
A. Bizzeti, 
P.M. Bj\o rnstad, 
T. Blake, 
F. Blanc, 
C. Blanks, 
J. Blouw, 
S. Blusk, 
A. Bobrov, 
V. Bocci, 
A. Bondar, 
N. Bondar, 
W. Bonivento, 
S. Borghi, 
A. Borgia, 
T.J.V. Bowcock, 
E. Bowen, 
C. Bozzi, 
T. Brambach, 
J. van den Brand, 
J. Bressieux, 
D. Brett, 
M. Britsch, 
T. Britton, 
N.H. Brook, 
H. Brown, 
I. Burducea, 
A. Bursche, 
J. Buytaert, 
S. Cadeddu, 
O. Callot, 
M. Calvi, 
M. Calvo Gomez, 
A. Camboni, 
P. Campana, 
A. Carbone, 
G. Carboni, 
R. Cardinale, 
A. Cardini, 
H. Carranza-Mejia, 
L. Carson, 
K. Carvalho Akiba, 
G. Casse, 
M. Cattaneo, 
Ch. Cauet, 
M. Charles, 
Ph. Charpentier, 
P. Chen, 
N. Chiapolini, 
M. Chrzaszcz , 
K. Ciba, 
X. Cid Vidal, 
G. Ciezarek, 
P.E.L. Clarke, 
M. Clemencic, 
H.V. Cliff, 
J. Closier, 
C. Coca, 
V. Coco, 
J. Cogan, 
E. Cogneras, 
P. Collins, 
A. Comerma-Montells, 
A. Contu, 
A. Cook, 
M. Coombes, 
G. Corti, 
B. Couturier, 
G.A. Cowan, 
D. Craik, 
S. Cunliffe, 
R. Currie, 
C. D'Ambrosio, 
P. David, 
P.N.Y. David, 
I. De Bonis, 
K. De Bruyn, 
S. De Capua, 
M. De Cian, 
J.M. De Miranda, 
L. De Paula, 
W. De Silva, 
P. De Simone, 
D. Decamp, 
M. Deckenhoff, 
H. Degaudenzi, 
L. Del Buono, 
C. Deplano, 
D. Derkach, 
O. Deschamps, 
F. Dettori, 
A. Di Canto, 
J. Dickens, 
H. Dijkstra, 
P. Diniz Batista, 
M. Dogaru, 
F. Domingo Bonal, 
S. Donleavy, 
F. Dordei, 
A. Dosil Su\'{a}rez, 
D. Dossett, 
A. Dovbnya, 
F. Dupertuis, 
R. Dzhelyadin, 
A. Dziurda, 
A. Dzyuba, 
S. Easo, 
U. Egede, 
V. Egorychev, 
S. Eidelman, 
D. van Eijk, 
S. Eisenhardt, 
U. Eitschberger, 
R. Ekelhof, 
L. Eklund, 
I. El Rifai, 
Ch. Elsasser, 
D. Elsby, 
A. Falabella, 
C. F\"{a}rber, 
G. Fardell, 
C. Farinelli, 
S. Farry, 
V. Fave, 
D. Ferguson, 
V. Fernandez Albor, 
F. Ferreira Rodrigues, 
M. Ferro-Luzzi, 
S. Filippov, 
C. Fitzpatrick, 
M. Fontana, 
F. Fontanelli, 
R. Forty, 
O. Francisco, 
M. Frank, 
C. Frei, 
M. Frosini, 
S. Furcas, 
E. Furfaro, 
A. Gallas Torreira, 
D. Galli, 
M. Gandelman, 
P. Gandini, 
Y. Gao, 
J. Garofoli, 
P. Garosi, 
J. Garra Tico, 
L. Garrido, 
C. Gaspar, 
R. Gauld, 
E. Gersabeck, 
M. Gersabeck, 
T. Gershon, 
Ph. Ghez, 
V. Gibson, 
V.V. Gligorov, 
C. G\"{o}bel, 
D. Golubkov, 
A. Golutvin, 
A. Gomes, 
H. Gordon, 
M. Grabalosa G\'{a}ndara, 
R. Graciani Diaz, 
L.A. Granado Cardoso, 
E. Graug\'{e}s, 
G. Graziani, 
A. Grecu, 
E. Greening, 
S. Gregson, 
O. Gr\"{u}nberg, 
B. Gui, 
E. Gushchin, 
Yu. Guz, 
T. Gys, 
C. Hadjivasiliou, 
G. Haefeli, 
C. Haen, 
S.C. Haines, 
S. Hall, 
T. Hampson, 
S. Hansmann-Menzemer, 
N. Harnew, 
S.T. Harnew, 
J. Harrison, 
P.F. Harrison, 
T. Hartmann, 
J. He, 
V. Heijne, 
K. Hennessy, 
P. Henrard, 
J.A. Hernando Morata, 
E. van Herwijnen, 
E. Hicks, 
D. Hill, 
M. Hoballah, 
C. Hombach, 
P. Hopchev, 
W. Hulsbergen, 
P. Hunt, 
T. Huse, 
N. Hussain, 
D. Hutchcroft, 
D. Hynds, 
V. Iakovenko, 
P. Ilten, 
R. Jacobsson, 
A. Jaeger, 
E. Jans, 
F. Jansen, 
P. Jaton, 
F. Jing, 
M. John, 
D. Johnson, 
C.R. Jones, 
B. Jost, 
M. Kaballo, 
S. Kandybei, 
M. Karacson, 
T.M. Karbach, 
I.R. Kenyon, 
U. Kerzel, 
T. Ketel, 
A. Keune, 
B. Khanji, 
O. Kochebina, 
I. Komarov, 
R.F. Koopman, 
P. Koppenburg, 
M. Korolev, 
A. Kozlinskiy, 
L. Kravchuk, 
K. Kreplin, 
M. Kreps, 
G. Krocker, 
P. Krokovny, 
F. Kruse, 
M. Kucharczyk, 
V. Kudryavtsev, 
T. Kvaratskheliya, 
V.N. La Thi, 
D. Lacarrere, 
G. Lafferty, 
A. Lai, 
D. Lambert, 
R.W. Lambert, 
E. Lanciotti, 
G. Lanfranchi, 
C. Langenbruch, 
T. Latham, 
C. Lazzeroni, 
R. Le Gac, 
J. van Leerdam, 
J.-P. Lees, 
R. Lef\`{e}vre, 
A. Leflat, 
J. Lefran\c{c}ois, 
O. Leroy, 
Y. Li, 
L. Li Gioi, 
M. Liles, 
R. Lindner, 
C. Linn, 
B. Liu, 
G. Liu, 
J. von Loeben, 
J.H. Lopes, 
E. Lopez Asamar, 
N. Lopez-March, 
H. Lu, 
J. Luisier, 
H. Luo, 
F. Machefert, 
I.V. Machikhiliyan, 
F. Maciuc, 
O. Maev, 
S. Malde, 
G. Manca, 
G. Mancinelli, 
N. Mangiafave, 
U. Marconi, 
R. M\"{a}rki, 
J. Marks, 
G. Martellotti, 
A. Martens, 
L. Martin, 
A. Mart\'{i}n S\'{a}nchez, 
M. Martinelli, 
D. Martinez Santos, 
D. Martins Tostes, 
A. Massafferri, 
R. Matev, 
Z. Mathe, 
C. Matteuzzi, 
M. Matveev, 
E. Maurice, 
A. Mazurov, 
J. McCarthy, 
R. McNulty, 
B. Meadows, 
F. Meier, 
M. Meissner, 
M. Merk, 
D.A. Milanes, 
M.-N. Minard, 
J. Molina Rodriguez, 
S. Monteil, 
D. Moran, 
P. Morawski, 
R. Mountain, 
I. Mous, 
F. Muheim, 
K. M\"{u}ller, 
R. Muresan, 
B. Muryn, 
B. Muster, 
P. Naik, 
T. Nakada, 
R. Nandakumar, 
I. Nasteva, 
M. Needham, 
N. Neufeld, 
A.D. Nguyen, 
T.D. Nguyen, 
C. Nguyen-Mau, 
M. Nicol, 
V. Niess, 
R. Niet, 
N. Nikitin, 
T. Nikodem, 
A. Nomerotski, 
A. Novoselov, 
A. Oblakowska-Mucha, 
V. Obraztsov, 
S. Oggero, 
S. Ogilvy, 
O. Okhrimenko, 
R. Oldeman, 
M. Orlandea, 
J.M. Otalora Goicochea, 
P. Owen, 
B.K. Pal, 
A. Palano, 
M. Palutan, 
J. Panman, 
A. Papanestis, 
M. Pappagallo, 
C. Parkes, 
C.J. Parkinson, 
G. Passaleva, 
G.D. Patel, 
M. Patel, 
G.N. Patrick, 
C. Patrignani, 
C. Pavel-Nicorescu, 
A. Pazos Alvarez, 
A. Pellegrino, 
G. Penso, 
M. Pepe Altarelli, 
S. Perazzini, 
D.L. Perego, 
E. Perez Trigo, 
A. P\'{e}rez-Calero Yzquierdo, 
P. Perret, 
M. Perrin-Terrin, 
G. Pessina, 
K. Petridis, 
A. Petrolini, 
A. Phan, 
E. Picatoste Olloqui, 
B. Pietrzyk, 
T. Pila\v{r}, 
D. Pinci, 
S. Playfer, 
M. Plo Casasus, 
F. Polci, 
G. Polok, 
A. Poluektov, 
E. Polycarpo, 
D. Popov, 
B. Popovici, 
C. Potterat, 
A. Powell, 
J. Prisciandaro, 
V. Pugatch, 
A. Puig Navarro, 
W. Qian, 
J.H. Rademacker, 
B. Rakotomiaramanana, 
M.S. Rangel, 
I. Raniuk, 
N. Rauschmayr, 
G. Raven, 
S. Redford, 
M.M. Reid, 
A.C. dos Reis, 
S. Ricciardi, 
A. Richards, 
K. Rinnert, 
V. Rives Molina, 
D.A. Roa Romero, 
P. Robbe, 
E. Rodrigues, 
P. Rodriguez Perez, 
G.J. Rogers, 
S. Roiser, 
V. Romanovsky, 
A. Romero Vidal, 
J. Rouvinet, 
T. Ruf, 
H. Ruiz, 
G. Sabatino, 
J.J. Saborido Silva, 
N. Sagidova, 
P. Sail, 
B. Saitta, 
C. Salzmann, 
B. Sanmartin Sedes, 
M. Sannino, 
R. Santacesaria, 
C. Santamarina Rios, 
E. Santovetti, 
M. Sapunov, 
A. Sarti, 
C. Satriano, 
A. Satta, 
M. Savrie, 
D. Savrina, 
P. Schaack, 
M. Schiller, 
H. Schindler, 
S. Schleich, 
M. Schlupp, 
M. Schmelling, 
B. Schmidt, 
O. Schneider, 
A. Schopper, 
M.-H. Schune, 
R. Schwemmer, 
B. Sciascia, 
A. Sciubba, 
M. Seco, 
A. Semennikov, 
K. Senderowska, 
I. Sepp, 
N. Serra, 
J. Serrano, 
P. Seyfert, 
M. Shapkin, 
I. Shapoval, 
P. Shatalov, 
Y. Shcheglov, 
T. Shears, 
L. Shekhtman, 
O. Shevchenko, 
V. Shevchenko, 
A. Shires, 
R. Silva Coutinho, 
T. Skwarnicki, 
N.A. Smith, 
E. Smith, 
M. Smith, 
K. Sobczak, 
M.D. Sokoloff, 
F.J.P. Soler, 
F. Soomro, 
D. Souza, 
B. Souza De Paula, 
B. Spaan, 
A. Sparkes, 
P. Spradlin, 
F. Stagni, 
S. Stahl, 
O. Steinkamp, 
S. Stoica, 
S. Stone, 
B. Storaci, 
M. Straticiuc, 
U. Straumann, 
V.K. Subbiah, 
S. Swientek, 
V. Syropoulos, 
M. Szczekowski, 
P. Szczypka, 
T. Szumlak, 
S. T'Jampens, 
M. Teklishyn, 
E. Teodorescu, 
F. Teubert, 
C. Thomas, 
E. Thomas, 
J. van Tilburg, 
V. Tisserand, 
M. Tobin, 
S. Tolk, 
D. Tonelli, 
S. Topp-Joergensen, 
N. Torr, 
E. Tournefier, 
S. Tourneur, 
M.T. Tran, 
M. Tresch, 
A. Tsaregorodtsev, 
P. Tsopelas, 
N. Tuning, 
M. Ubeda Garcia, 
A. Ukleja, 
D. Urner, 
U. Uwer, 
V. Vagnoni, 
G. Valenti, 
R. Vazquez Gomez, 
P. Vazquez Regueiro, 
S. Vecchi, 
J.J. Velthuis, 
M. Veltri, 
G. Veneziano, 
M. Vesterinen, 
B. Viaud, 
D. Vieira, 
X. Vilasis-Cardona, 
A. Vollhardt, 
D. Volyanskyy, 
D. Voong, 
A. Vorobyev, 
V. Vorobyev, 
C. Vo\ss, 
H. Voss, 
R. Waldi, 
R. Wallace, 
S. Wandernoth, 
J. Wang, 
D.R. Ward, 
N.K. Watson, 
A.D. Webber, 
D. Websdale, 
M. Whitehead, 
J. Wicht, 
J. Wiechczynski, 
D. Wiedner, 
L. Wiggers, 
G. Wilkinson, 
M.P. Williams, 
M. Williams, 
F.F. Wilson, 
J. Wishahi, 
M. Witek, 
S.A. Wotton, 
S. Wright, 
S. Wu, 
K. Wyllie, 
Y. Xie, 
F. Xing, 
Z. Xing, 
Z. Yang, 
R. Young, 
X. Yuan, 
O. Yushchenko, 
M. Zangoli, 
M. Zavertyaev, 
F. Zhang, 
L. Zhang, 
W.C. Zhang, 
Y. Zhang, 
A. Zhelezov, 
A. Zhokhov, 
L. Zhong, 
A. Zvyagin

